A minimal model for finite temperature superfluid dynamics

Building on a recently improved understanding of the problem of heat flow in general relativity, we develop a hydrodynamical model for coupled finite temperature superfluids. The formalism is designed with the dynamics of the outer core of a mature neutron star (where superfluid neutrons are coupled to a conglomerate of protons and electrons) in mind, but the main ingredients are relevant for a range of analogous problems. The entrainment between material fluid components (the condensates) and the entropy (the thermal excitations) plays a central role in the development. We compare and contrast the new model to previous results in the literature, and provide estimates for the relevant entrainment coefficients that should prove useful in future applications. Finally, we consider the sound-wave propagation in the system in two simple limits, demonstrating the presence of second sound if the temperature is sub-critical, but absence of this phenomenon above the critical temperature for superfluidity.

==> PaxHeader/SFthermalv3.tex <==
18 gid=1338971407
17 uid=423933575
20 ctime=1355751036
20 atime=1355751038
38 LIBARCHIVE.creationtime=1350060840
23 SCHILY.dev=16777218
22 SCHILY.ino=6276344
18 SCHILY.nlink=1

